CodeFlow: Program Behavior Prediction with Dynamic Dependencies Learning

Predicting program behavior without execution is a critical task in software engineering. Existing models often fall short in capturing the dynamic dependencies among program elements. To address this, we present CodeFlow, a novel machine learning-based approach that predicts code coverage and detects runtime errors by learning both static and dynamic dependencies within the code. By using control flow graphs (CFGs), CodeFlow effectively represents all possible execution paths and the statistic relations between different statements, providing a more comprehensive understanding of program behaviors. CodeFlow constructs CFGs to represent possible execution paths and learns vector representations (embeddings) for CFG nodes, capturing static control-flow dependencies. Additionally, it learns dynamic dependencies by leveraging execution traces, which reflect the impacts among statements during execution. This combination enables CodeFlow to accurately predict code coverage and identify runtime errors. Our empirical evaluation demonstrates that CodeFlow significantly improves code coverage prediction accuracy and effectively localizes runtime errors, outperforming state-of-the-art models.

==> generalisation.tex <==
\section{Runtime Error Detection Accuracy [RQ2]}

In this RQ, we evaluate {\tool}'s generalization capability. This aims to determine how well it performs when trained on shorter code snippets but tested on more complex code.

\subsection{Data Collection}
For this evaluation, we generated a new synthetic dataset containing approximately 1,200 Python code snippets for testing out trained model. Each snippet consists of 70-100 lines of code, significantly longer and more complex than the original dataset, which contained snippets of 5-20 lines. The new dataset is designed to cover a wide range of programming constructs and execution paths to test the robustness and generalization of {\tool} effectively.

\subsection{Empirical Results}
We assessed the performance of {\tool} on the new testset using the same metrics as in RQ1: Exact Matching, Branching Correctness, Precision, Recall, and F1-Score. The results are presented in Table~\ref{tab:generalization}.

\begin{table}[!h]
\centering
\caption{Generalization Performance of {\tool} on Longer Code Snippets in New Dataset}
\label{tab:generalization}
\begin{adjustbox}{width=0.49\textwidth}
\begin{tabular}{@{}lccccc@{}}
\toprule
Dataset & Match & Branch & Precision & Recall & F1-Score \\ \midrule
Original Testset & 75.24\% & 87.88\% & 0.97 & 0.97 & 0.97 \\ 
New Testset & 71.47\% & 82.56\% & 0.94 & 0.92 & 0.93 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

The results indicate that {\tool} maintains its high performance even when evaluated on longer and more complex code snippets. The exact matching accuracy of {\tool} on the new dataset is \textbf{71.47\%}, which is slightly lower than the 75.24\% achieved on the original dataset but still demonstrates strong performance. This slight reduction is expected due to the increased complexity and length of the new code snippets.

\begin{table*}[!h]
\centering
\caption{Runtime Error Localization Accuracy of {\tool}}
\label{tab:runtime_error_results}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}{*}{Metric} & \multicolumn{2}{c}{Code Executor} & \multicolumn{2}{c}{LLM} & \multicolumn{2}{c}{XYZ (Our)} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
& Complete Dataset & Incomplete Dataset & Complete Dataset & Incomplete Dataset & Complete Dataset & Incomplete Dataset \\ \midrule
Runtime Error Detection Acc &  &  &  &  & 97.51\% & 97.53\% \\ 
Bug Localization Acc &  &  &  &  & 72.22\% & 70.30\% \\ 
Exact Matching &  &  &  &  & 72.77\% & 72.87\% \\ 
Branching Correctness &  &  &  &  & 83.10\% & 81.94\% \\ 
Precision &  &  &  &  & 0.96 & 0.95 \\ 
Recall &  &  &  &  & 0.97 & 0.97 \\ 
F1 Score &  &  &  &  & 0.96 & 0.96 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

Branching correctness remains high at \textbf{82.56\%}, compared to 87.88\% on the original dataset. This indicates that {\tool} continues to accurately predict which branches are executed after conditional statements, even in longer and more complex code.

Precision and recall are also slightly lower on the new dataset, with precision at 0.94 and recall at 0.92, compared to 0.97 for both on the original dataset. The F1-Score, which balances precision and recall, is 0.93 on the new dataset, slightly lower than the 0.97 on the original dataset.
